The Inverse Problem of Reconstructing Reaction-Diffusion Systems

This paper considers the inverse problem of recovering state-dependent source terms in a reaction-diffusion system from overposed data consisting of the values of the state variables either at a fixed finite time (census-type data) or a time trace of their values at a fixed point on the boundary of the spatial domain. We show both uniqueness results and the convergence of an iteration scheme designed to recover these sources. This leads to a reconstructive method and we shall demonstrate its effectiveness by several illustrative examples.

==> recon_fig_legend.tex <==
\newbox\figurelegendtwo
\newdimen\xxfiglen \newdimen\yyfiglen
\xxfiglen=0.5true in
\yyfiglen=0.1true in
%
\setbox\figurelegendtwo=\hbox{
\beginpicture
  \setcoordinatesystem units <\xxfiglen,\yyfiglen> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 5
\footnotesize
\linethickness=0.7pt
\eightrm
   \setdashes <3pt>  \putrule from 0 5 to 0.75 5
   \setsolid
   \Goldenrod{\relax\putrule from 0 4 to 0.75 4 \relax}\relax
   \Orange{\relax\putrule from 0 3 to 0.75 3 \relax}\relax
   \Red{\relax\putrule from 0 2 to 0.75 2 \relax}\relax
   \LimeGreen{\relax\putrule from 0 1 to 0.75 1 \relax}\relax
   \PineGreen{\relax\putrule from 0 0 to 0.75 0 \relax}\relax
  \setsolid
  \put {$f_{\hbox{act}}$}  [lb] at 1 5
  \put {${\hbox{iter}\,1}$}  [l] at 1 4
  \put {$_{\hbox{iter}\,2}$}  [l] at 1 3
  \put {$_{\hbox{iter}\,3}$} [l] at 1 2
  \put {$_{\hbox{iter}\,5}$} [l] at 1 1
  \put {$_{\hbox{iter}\,10}$} [l] at 1 0
\endpicture
}
%


